Empowering Distributed Training with Sparsity-driven Data Synchronization

Distributed training is the de facto standard to scale up the training of deep learning models with multiple GPUs. Its performance bottleneck lies in communications for gradient synchronization. Although high tensor sparsity is widely observed, the optimal communication scheme to fully leverage sparsity is still missing. This paper aims to bridge this gap. We first analyze the characteristics of sparse tensors in popular models to understand the fundamentals of sparsity. We then systematically explore the design space of communication schemes for sparse tensors and find the optimal ones. These findings give a new understanding and inspire us to develop a holistic gradient synchronization system called Zen for sparse tensors. We demonstrate that Zen can achieve up to 5.09x speedup in communication time and up to $2.48\times$ speedup in training throughput compared to the state-of-the-art methods.

==> background.tex <==
\section{Background}

\subsection{Distributed DNN Training}\label{sec:background_dnn}
Deep Neural Networks~(DNN) have demonstrated superior empirical performance in most artificial intelligence applications~\cite{sundermeyer2012lstm, guo2017deepfm, he2017neural, bert, opt175b}. The standard training procedure of DNN consists of three steps. Firstly, given a batch of input samples, it computes the DNN predictions through \textit{forward propagation} and compares them with the labels to get losses. 
Secondly, it performs \textit{back-propagation} from the last layer towards the first layer to obtain the gradient of each parameter. 
Thirdly, it updates each parameter using the computed gradient. 
The gradients of the parameters in a specific DNN layer form a \textit{tensor}.

To accelerate training of DNN models on massive datasets, the most popular paradigm is data-parallel distributed training~(DDT)~\cite{dean2012large, PSosdi2014, horovod, byteps_osdi, pytorch_ddp}. 
In this paradigm, the training dataset is partitioned and allocated to multiple graphics processing units~(GPUs). 
In each iteration, each GPU computes its own gradients using a batch sampled from its assigned partition. 
Since the batch for each GPU is different, the gradient tensors generated by back-propagation will also be different.
DDT requires aggregation and synchronization of the gradient tensors from all GPUs to ensure model consistency.

% AllReduce~\cite{tensorflow, pytorch_ddp, horovod, NCCL} is widely used for gradient synchronization in DDT.
% It is proved to be bandwidth optimal given a set of GPU machines~\cite{patarasuk2009bandwidth}.
% BytePS~\cite{byteps_osdi} can outperform Allreduce when a training system has additional CPU machines and bandwidth resources for gradient synchronization.
% Unfortunately, both Allreduce and BytePS disregard the values of gradients and communicate all gradients in a tensor even if they are mostly zeros.

\subsection{Sparsity in DNN Models}
\label{sec:motivate_sparsity}

\begin{table*}[ht]
\footnotesize
\centering
\begin{tabular}{ccccccc}
\hline
Model  & Task & Dataset & MLP Gradient Size & Embedding Gradient Size & Batch Size & Density  \\
\hline \hline
LSTM  & Language Modeling & One Billion Word & 20M & 406M & 128 &	 $1.13\%$ \\
DeepFM  & Click-through Rate Prediction &   Criteo & 68M &	214M & 1024 &	 $2.80\%$ \\
% NCF   & Collaborative Filtering & Yelp & 10M	& 132M 	& 16 & $0.06\%$		\\
NMT  &Machine Translation & IWSLT 2014 De-En &	31M &	112M & 64 & $2.47\%$ 	\\
BERT  & Question Answering & SQuAD v1.1 & 86M	& 23M	& 4 &	$1.06\%$ \\
\hline
\end{tabular}
\vspace{-0.1in}
\caption{DNN models and their training statistics. Density is the average density of embedding gradient tensors on a single GPU.}
\label{tab:model_sparsity}
\vspace{-0.1in}
\end{table*}

The most popular paradigm to accelerate training of DNN models on massive datasets is data-parallel distributed training~(DDT)~\cite{dean2012large, PSosdi2014, horovod, byteps_osdi, pytorch_ddp}. 
In this paradigm, the training dataset is partitioned and allocated to multiple GPUs. 
In each iteration, each GPU computes its own gradients using a batch sampled from its assigned partition. 
Since the batch for each GPU is different, the gradient tensors generated in different GPUs will also be different.
DDT requires aggregation and synchronization of the gradient tensors from all GPUs to ensure model consistency.


% Recently, practitioners from the deep learning community have observed and explored the sparsity in gradient tensors~\cite{chen2020slide,medini2020solar,clp+21,wang2022dragonn}. 
Because the training procedure of DNN models may focus on updating a subset of parameters instead of all of them~\cite{frankle2018lottery,you2020drawing}, some of the gradient tensors in DNN models are naturally sparse, with most of the gradients being zeros. 
Table~\ref{tab:model_sparsity} lists the statistics of four widely-deployed DNN models for both recommendations systems and language processing.
Each model contains two parts: multilayer perceptron~(MLP) and embedding table.
There are two major observations from Table~\ref{tab:model_sparsity}.
Firstly, the embedding tables comprise a large portion of model parameters. 
Secondly, these embedding tables show a significant level of sparsity in their gradient tensors. 
We define the \textit{density} of a gradient tensor as the percentage of its non-zero gradient values and then provide the average density for the sparse gradient tensors in the four models. 
As shown in the table, gradient tensors can have only $1.06\%$ non-zero gradients in DNN training.

If the notable sparsity can be leveraged, it can significantly reduce the traffic volume for gradient synchronization and shorten the communication time in DDT.
Previous works~\cite{kim2019parallax, omnireduce, sparcml} have recognized this potential, but the fundamental implications of sparsity are not yet understood.

==> implementation.tex <==
\section{Implementation}

We implement {\name} with Horovod~\cite{horovod}, a popular DDT framework to support the gradient synchronization of DNN training jobs.
We also leverage DistributedDataParallel (DDP) in PyTorch to implement hierarchical communication for sparse tensors.


\noindent
\textbf{Hashing with GPUs.}
{\name} performs Algorithm~\ref{alg:hash} on GPUs to load balance sparse tensors for communication because GPUs are much faster than CPUs for the implementation.
One concern to use GPUs is that it competes for the GPU resource with back-propagation and thus delays the training process~\cite{agarwal2021utility}.
Fortunately, because the sparsity typically comes from the embedding table, which is the first layer of a DNN model, its gradients are computed at the end of back-propagation.
There is almost no GPU resource competition between load balancing sparse tensors and back-propagation.

\noindent
\textbf{Hash functions.}


